Generating Formal Safety Assurances for High-Dimensional Reachability

Providing formal safety and performance guarantees for autonomous systems is becoming increasingly important. Hamilton-Jacobi (HJ) reachability analysis is a popular formal verification tool for providing these guarantees, since it can handle general nonlinear system dynamics, bounded adversarial system disturbances, and state and input constraints. However, it involves solving a PDE, whose computational and memory complexity scales exponentially with respect to the state dimensionality, making its direct use on large-scale systems intractable. A recently proposed method called DeepReach overcomes this challenge by leveraging a sinusoidal neural PDE solver for high-dimensional reachability problems, whose computational requirements scale with the complexity of the underlying reachable tube rather than the state space dimension. Unfortunately, neural networks can make errors and thus the computed solution may not be safe, which falls short of achieving our overarching goal to provide formal safety assurances. In this work, we propose a method to compute an error bound for the DeepReach solution. This error bound can then be used for reachable tube correction, resulting in a safe approximation of the true reachable tube. We also propose a scenario-based optimization approach to compute a probabilistic bound on this error correction for general nonlinear dynamical systems. We demonstrate the efficacy of the proposed approach in obtaining probabilistically safe reachable tubes for high-dimensional rocket-landing and multi-vehicle collision-avoidance problems.

==> initial_sub/sections/intro.tex <==
\section{Introduction}
Imagine the real-world motivating example of an aerial vehicle that wants to reach a destination while avoiding any collisions. There might even be adversarial disturbances, such as wind or another aircraft nearby, that have the potential to hinder the vehicle from achieving its objective. Since such autonomous systems are becoming increasingly common in our everyday lives, it is vital that we can compute controllers with provable safety guarantees. There already exist many approaches in the literature for computing these. For example, ... However, they are limited by ... The popular Hamilton-Jacobi reachability approach, on the other hand, addresses many of these limitations.

\textbf{Hamilton-Jacobi Reachability Methods.} Hamilton-Jacobi (HJ) reachability analysis is a popular formal verification method for autonomous systems that computes both a safe controller and its corresponding safe state configurations. Its advantages over other approaches includes its ability to handle general nonlinear system dynamics, bounded adversarial system disturbances, and state and input constraints. 

In reachability analysis, we are interested in the \textit{Backward Reachable Tube (BRT)} of a dynamical system, which is defined in the following Section \ref{sec:problem_setup} in Equation \eqref{eq:reachBRT}, since it directly relates to system safety.
Hamilton-Jacobi reachability analysis computes a system's BRT by solving a Hamilton-Jacobi (HJ) partial differential equation (PDE) \eqref{eq:HJIVI}, as explained in Section \ref{sec:problem_setup}. Level set methods can compute BRTs accurately up to numerical precision on a grid representing a discretization of the state space \cite{mitchell2005time, lygeros2004reachability, Margellos11, fisac2015reach, bansal2017hamilton}.
Unfortunately, this process results in an exponential scaling of memory and computational complexity with respect to system dimensionality, making it challenging to scale beyond 5D systems \cite{bansal2017hamilton}.

Several methods have been proposed to overcome this challenge by trading off between the class of dynamics they can handle, the approximation quality of the BRT, and the required computation. For example, the methods presented in \cite{Greenstreet1998, Frehse2011, Kurzhanski00, Kurzhanski02, Maidens13, girard2005reachability, althoff2010computing} analyze high-dimensional affine systems using sets of pre-specified shapes, sum-of-squares optimization \cite{Majumdar13, majumdar2017funnel} and parallelotopes \cite{Dreossi16} rely on specific dynamics for computing BRTs for polynomial dynamics \cite{henrion2014convex}; leverage monotonicity of dynamics \cite{coogan2015efficient}; use decoupled or reduced order dynamics to decompose the BRT computation \cite{chen2018decomposition, holmes2020reachable, liu2020leveraging, Chen2016d, somil2020sequential}; leverage the Hopf-Lax formula to compute BRTs for convex dynamics \cite{chow2017algorithm}; or deal with affine dynamics \cite{bak2019numerical, Nilsson2016}.
Control Lyapunov (and Barrier) functions are also used to design safety controller \cite{ames2016control, ames2019control}; however, finding feasible Lyapunov functions can be challenging, especially in the presence of control or disturbance bounds.

Sampling and learning-based methods have also been explored for computing BRTs \cite{liebenwein2018sampling}, including scenario optimization \cite{sutter2017data, devonport2020estimating, ghosh2019new} and adversarial sampling \cite{lew2020sampling}, Support Vector Machines \cite{allen2014machine} and DNNs \cite{rubies2019classification, fisac2019bridging, darbon2020overcoming, niarchos2006neural, djeridane2006neural} leveraging data to compute approximate BRTs for nonlinear systems; however, they often struggle in the presence of adversarial disturbances and state constraints.
Other methods require explicit supervision for learning which is hard to generate for general high-dimensional systems.

Unfortunately, all these methods either need strong assumptions on dynamics, cannot handle presence of exogenous inputs or hard constraints, or lead to a very conservative approximation of the reachable set.
Additionally, very few of these approaches can handle adversarial inputs; yet, considering adversarial inputs (e.g., other agents or the model uncertainty) and state constraints is critical in analysis 
and synthesis of safe controllers. Thus, in this work, we focus on a recently developed deep learning-based approach to approximately solve high-dimensional Hamilton-Jacobi reachability problems: \metName{}, which overcomes all of these limitations.

\textbf{DeepReach.} What sets \metName{} apart is its ability to compute BRTs as well as the \textit{corresponding safety controller} for \textit{general} nonlinear dynamical systems in the presence of \textit{disturbances} and \textit{state and input constraints}. 
In contrast to level-set methods, DeepReach learns continuous, rather than discretized, solutions to high-dimensional systems which would otherwise be intractable. 

Instead of solving this PDE over a grid, \metName{} draws inspiration from the recent progress in solving PDEs using deep learning, and represents the value function as a sinusoidal deep neural network (DNN) to learn a parameterized approximation of the value function via self-supervision on the PDE. 
\metName{} can also be interpreted as an approximate dynamic programming method \cite{bertsekas1995dynamic} where a DNN is used to \textit{learn} the basis features for the value function. 
Thus, the computation and memory requirements for obtaining the value function do not scale with the grid resolution, but rather the complexity of the value function.
This enables \metName{} to scale to general, high-dimensional dynamical systems.

Even if we can now obtain an approximate BRT for high-dimensional systems for the first time with DeepReach, they are limited in usefulness by their approximate nature. Recall that one of the primary use cases of Hamilton-Jacobi reachability is to provide formal, not approximate, safety guarantees. Thus, our work bridges this gap by proposing a verification method to transform a DeepReach solution into a formal guarantee.

\textbf{Existing Verification Methods.}

\textbf{\approachName{} Method.} 
\begin{enumerate}
    \item list specific contributions of this work
\end{enumerate}
%in this work, we want to bridge this gap by providing high confidence BRT tube: start explaining my own work, one-line summary of what I'm trying to do "we are trying to fill this gap", then next sentence is "our key idea is: find consistency between value and policy, use that gap as a signal to find ", then "this is a good idea because.. and it helps our main goal in a few sentences", then take a few more sentences to explain work further if needed. then quick sentences on how we validate or measure our work. We demonstrate the effectiveness of the scenario optimization approach, as well as the increased performance from auto-partitioning, on a series of increasingly challenging reachability safety problems. We start with a simple 3D system which can be solved by traditional level set methods that we compare to and progress to high-dimensional systems which are intractable to traditional level set methods. Thus, we produce safety guarantees on continuous resolution solutions which previously have been extremely difficult if not impossible to produce prior to this work (important contribution).

%This running example is chosen because it is simple to understand. Furthermore, it is a low-dimensional problem so a ground truth solution can be computed by level set methods. Later, we will validate the correctness of our verification method by comparing our recovered safety solution to the ground truth. 

